Differentially Private Data Analysis of Social Networks via Restricted Sensitivity

We introduce the notion of restricted sensitivity as an alternative to global and smooth sensitivity to improve accuracy in differentially private data analysis. The definition of restricted sensitivity is similar to that of global sensitivity except that instead of quantifying over all possible datasets, we take advantage of any beliefs about the dataset that a querier may have, to quantify over a restricted class of datasets. Specifically, given a query f and a hypothesis H about the structure of a dataset D, we show generically how to transform f into a new query f_H whose global sensitivity (over all datasets including those that do not satisfy H) matches the restricted sensitivity of the query f. Moreover, if the belief of the querier is correct (i.e., D is in H) then f_H(D) = f(D). If the belief is incorrect, then f_H(D) may be inaccurate. We demonstrate the usefulness of this notion by considering the task of answering queries regarding social-networks, which we model as a combination of a graph and a labeling of its vertices. In particular, while our generic procedure is computationally inefficient, for the specific definition of H as graphs of bounded degree, we exhibit efficient ways of constructing f_H using different projection-based techniques. We then analyze two important query classes: subgraph counting queries (e.g., number of triangles) and local profile queries (e.g., number of people who know a spy and a computer-scientist who know each other). We demonstrate that the restricted sensitivity of such queries can be significantly lower than their smooth sensitivity. Thus, using restricted sensitivity we can maintain privacy whether or not D is in H, while providing more accurate results in the event that H holds true.

==> itcs_abstract.tex <==
\begin{abstract}
We introduce the notion of {\em restricted sensitivity} as an alternative to
global and smooth sensitivity, in order to improve accuracy in differentially private data analysis.  The definition of restricted sensitivity is similar to that of global sensitivity except that instead of quantifying over all possible data sets, we a-priori postulate that our input belongs to a predefined set $\mathcal{H}$ of nice databases and quantify only over databases in this restricted set. In a computationally unbounded setting, we show that the querier may specify a query $f$ and a set $\mathcal{H}$ and we can devise a function $f_\mathcal{H}$ that identifies with $f$ over $\mathcal{H}$, and has its global sensitivity identical to the restricted sensitivity of $f$ over $\mathcal{H}$. Applying classical Laplacian mechanism to $f_{\cal H}$ preserves the privacy of any database, while guaranteeing good utility for databases in ${\cal H}$.
 
We demonstrate the usefulness of this notion by considering the task of answering queries regarding social-networks, which we model as a combination of a graph and a labeling of its vertices. For the specific definition of $\mathcal{H}$ as graphs of bounded degree, we exhibit efficient ways of deriving $f_{\cal H}$ using various projection-based techniques. We then discuss \emph{subgraph counting queries} (e.g., number of triangles) and \emph{local profile queries} (e.g., number of people who know a doctor), 
and demonstrate that the restricted sensitivity of such queries can be significantly lower than their smooth sensitivity.
\end{abstract}


==> itcs_definitions.tex <==


\section{ Definitions}
 \label{sec:Query} 
To overcome these challenges we introduce the notion of restricted sensitivity, using a hypothesis about the dataset $\mathcal{D}$ to restrict the sensitivity of a query. A hypothesis $H$ is a subset of the set of possible datasets -  $H \subseteq \mathcal{D}$ (in the context of a labeled graph $H \subseteq \mathcal{G}$). We say that a hypothesis $H$ is true if the true dataset $D \in H$. Because the hypothesis $H$ may not be a convex set we must consider all pairs of datasets in $H$ instead of all pairs of adjacent datasets as in the definition of global sensitivity.

\begin{definition} \label{def:RestrictedSensitivity}
The {\em restricted sensitivity} of $f$ given a hypothesis $H \subset \mathcal{D}$ is 
\[ RS_f\paren{H} = \max_{D_1,D_2 \in H} \frac{\abs{f\paren{D_1}-f\paren{D_2}}}{d\paren{G_1,G_2}} \ .\] 
\end{definition}

Observe that the $RS_f\paren{H}$ may be smaller than $LS_f\paren{D}$ for some $D \in H$ if $D$ could has a neighbor $D' \notin H$. In fact we often have \[LS_f\paren{D} \geq \left| f\paren{D} -f\paren{D'} \right| \gg RS_f\paren{H} \ .\]
In this case $RS_f\paren{H}$ will be significantly lower than $S_{f,\beta}\paren{D}$, an upper bound on $LS_f\paren{D}$, because smoothed sensitivity does not use the hypothesis $H$ to reduce the sensitivity. In general the mechanism $A\paren{D} = f\paren{D} + Lap\paren{RS_f\paren{H}/\epsilon}$ does not preserve differential privacy. To achieve differential privacy while adding noise proportional to $RS_f\paren{H}$ we must be willing to sacrifice accuracy guarantees for datasets $D \notin H$. Our goal is to create a new query $f_H$ such that  $f_H(D) = f(D)$ for every $D \in \mathcal{D}$ ($f_H$ is accurate when the hypothesis is correct) and $f_H$ either has 1) low global sensitivity or 2) low $\beta$-smooth sensitivity over datasets $D \in \mathcal{D}$. If we want an efficient mechanism in the second case then we must also be able to compute the smoothed sensitivity of $f_H$ efficiently.

We focus on the hypothesis $H_k = \{ G ~|~\Delta_G \leq k\}$, where $\Delta_G$ is the maximum vertex degree in the labeled graph $G$ (see definition \ref{def:SocialNetwork}). In many labeled graphs reasonable to believe that $H_k$ holds for $k \ll n$ because the degree distributions follow a power law. For example, the number of telephone numbers recieving $t$ calls in a day is proportional to $1/t^2$, and the number of web pages with $t$ incoming links is proportional to $1/t^2$ \cite{newman2003structure,broder2000graph,easley2010networks}. For these networks it would suffice to set $k = O\paren{\sqrt{n}}$. The number of papers that recieve $t$ citations is proportional to $1/t^3$ so we could set $k = O\paren{\sqrt[3]{n}}$ \cite{easley2010networks}. While the degrees on facebook don't seem to follow a power law, the upper bound $k=5,000$ seems reasonable \cite{ugander2011anatomy}. By contrast, facebook had approximately $n=901,000,000$ users in June, 2012 $(n>k^3)$ \cite{facebookStatistics}.

Our work is motivated by the challenges posed by differentially private analysis of social networks. Formally, we model a social network as a labeled graph. 
\begin{definition} \label{def:SocialNetwork}
A {\em labeled graph}  $G \in \mathcal{G}$ is a graph with labeling function $\ell:V \rightarrow C$ mapping vertices to attributes.  
\end{definition}
The labeling function $\ell$ allows us to encode information about the nodes (e.g., age, gender, occupation etc...). A labeled graph could be used to reprsesent a social network like facebook, a telephone call network, a collaboration network, etc...

Defining differential privacy over the labeled graphs $\mathcal{G}$ requires care. What does it mean for two labeled graphs $G_1, G_2 \in \mathcal{G}$ to be neighbors? There are two natural notions:

\begin{definition}
\label{def_Privacy:EdgeChanges} Edge Adjacency: We say that two graphs $G_1$ and $G_2$ are neighbors if 1. $\forall v, \ell_1(v) = \ell_2\paren{v}$ and $\abs{E_1  \vartriangle E_2 } = 1$ or 2. $\abs{E_1 \vartriangle E_2 } = 0$ and $\ell_1\paren{v} = \ell_2\paren{v}$ for every vertex except one. 
\end{definition}

In the context of a social network the privacy guarantees of differential-privacy wrt edge changes may not be very strong for an individual node $v$. An adversary may not be able to distinguish between graphs $G_1$ - in which node $v$ is connected to one criminals - and $G_2$ - in which node $v$ is connected to no criminals, but an adversary may be able to successfully distinguish between $G_2$ and $G_3$ - a graph in which node $v$ is connected to many criminals. By contrast, in the vertex adjacency model of differential privacy an adversary would not be able to distinguish the two graphs because $G_2$ and $G_3$ would be neighbors.

\begin{definition} \label{def_Privacy:VertexChanges} Vertex Adjacency: We say that two graphs $G_1$ and $G_2$ are neighbors if $\exists v'\in V$ such that $G_1 - v' = G_2-v'$ and $\forall v \in V-v', \ell_1\paren{v} = \ell_2\paren{v}$.
\end{definition}

Fixing a notion of adjacency we use $d\paren{G,G'}$ to denote the distance between two labeled graphs, and we use $d\paren{G,H}$ to denote the distance between $G$ and the closest graph in $H$.

The smoothed sensitivity of a query $f$ may be prohibitively large even for graphs $G \in H_k$. For example, let $f\paren{G} =$ ``the number of people in $G$ that are either 1) a democrat or 2) connected to at least one democrats?" has  $GS_f \geq n$ (consider two neighboring complete graphs $G$ and $G'$ where $G$ has no democrats - $f(G) = 0$ and $G'$ has exactly one democrats $f(G') = n$). Notice that the same basic example applies to {\em both} the edge adjacency and the vertex adjacency model. The laplacian mechanism could not be used to accurately answer the query $f$ while preserving $\epsilon$-differential privacy because the noise would be proportinal to $n/\epsilon$. By contrast, the restricted sensitivity of this query is at most $RS_f\paren{H_k} \leq 2k+1$.

Before we introduce subgraph counting queries and local profile queries it is necessary to introduce some notation. Let $G\left[v_i,..,v_k\right]$ be the subgraph induced by $v_i,...,v_k$ and let $N_v = \{v\} \cup \{x~|~\{x,v\} \in E(G)\}$ be the neighborhood of $v$. A profile $p: V \times \mathcal{G} \rightarrow [0,1]$ is a function which take a vertex $v$ and a graph $G$. The value of a local profile query $p(v,G)$ depends only on $N_v$, the local neighborhood  of $v$. We adopt the notaion $p\paren{v,N_v}$ for convenience.

\begin{definition}\label{query:SubgraphCounting} 
 Given a constant-sized labeled subgraph $P$ and a labled graph $G$, a subgraph counting query $f^P(G)$ asks how many copies of $P$ appear in $G$. Formally queries have the form, $ f^P\left(G\right) = \left| S_{P,G}\right|$,  where
 \[S_{P,G} = \{\{v_{i_1},...,v_{i_{|P|}}\}~\vline ~P = G\left[v_{i_1},...,v_{i_{|P|}}\right] \} \ . \]  
\end{definition}

For example, a researcher may be interested in learning how many triangles $(P=K_3)$ are in the graph. The smooth-sensitivity of $f^{K_3}$ can be computed efficiently in the edge-adjacency model for unlabed graphs \cite{KRSY11}. In the appendix we show how to efficiently compute the $\beta$-smooth sensitivity in the vertex-adjacency model. Claims \ref{claim:SmoothSensitivitySubgraphCounting} and \ref{claim:RestrictedSensitivitySubgraphCounting} demonstrate that the $\beta$-smooth sensitivity is much higher than the restricted sensitivity under the hypothesis $H_k$ whenever $k \ll n$.

\begin{definition} \label{query:NodesWithProfile} A {\em (local) profile query} $f_p$ sums the (local) profile  $p$ accross all  nodes
\[f_p\left(G\right) = \sum_{v \in V(G)} p\left(v,G\right) \ . \] 

\end{definition}

The restricted sensitivity of a local profile query given the hypothesis $H_k$ is $RS_f\paren{H_k} \leq k+1$ in the edge adjacency model (e.g., by changing its label a node $v$ can affect the profile of itself and all $k$ of its neighbors).  In the vertex adjacency model the restricted sensitivity is at most $RS_f\paren{H_k} \leq 2k+1$ (e.g., by changing its neighbors a node $v$ can affect the local profiles of itself, its $k$ old neighbors and its $k$ new neighbors). See claim \ref{claim:RestrictedSensitivityLocalProfileQuery} for a more rigorous proof.

Local profiles are an . For example, the clustering coefficient $c(v)$ \cite{watts1998collective,newman2003structure} of a node $v$ is the probability that two randomly selected friends are friends with each other. The clustering coefficient has been used to identify teenage girls who are more likely to consider suicide\cite{bearman2004suicide}. One explanation, is that it becomes an inherent source of stress if two friends are not friends with each other \cite{easley2010networks}. Notice that the average clustering coefficient $\paren{\sum_v c\paren{v}}$ is an example of local profile query. The average clustering coefficient of a graph can also be computed from $f^{K_3}$ and $f^{2-Star}$. Bridges are another example of an interesting query captured by local profiles. An edge $\{x,y\}$ is a local bridge if its endpoints have no friends in common. Bridges ``provide their endpoints with access to parts of the network - and hence sources of information - that they would otherwise be far away from \cite{easley2010networks}." For example, a 1995 study showed that the best job leads often come from aquaintances rather than close friends \cite{granovetter1995getting}. We might call a node $x$ `influential' if  many incident edges are bridges. A marketing agency may be interested in identifying groups of people that are influential. 

We say that the $2$-betweeness of a vertex $v$ is the probability that the a randomly chosen shortest path between two randomly chosen neighbors $x,y \in N_v$ goes through $v$. Betweeness \cite{freeman1979centrality} can also be used to measure the influence of a node $x$.



==> itcs_introduction.tex <==
\section{Introduction}

Social networks have been the subject of much research~(see the survey book of~\cite{easley2010networks}), and the fact that the data in a social network might be used to infer sensitive details about an individual, like sexual orientation \cite{jernigan2009gaydar}, is a growing concern among social networks' participants. Even in an `anonymized' unlabeled graph it is possible to identify people based on graph structures \cite{backstrom2007wherefore}. And yet there has been very little work relating the rigorous framework of differential privacy~\cite{dwork2006differential,Dwork06calibratingnoise} to the field of social networks. 

Indeed, there are intrinsic difficulties when applying differential privacy to social networks' analysis. Differential privacy requires that for any network, any change to a single person will only cause a very limited change to the algorithm's distribution over outputs. Yet it is simple to see that many potentially interesting graph-queries are highly sensitive to the change caused by a single node. (E.g. in a complete bipartite graph a single node may connect to all other nodes thus increasing the number of triangles from $0$ to $\Omega(n^2)$.) In concrete terms -- if we allow a vertex to change all of the edges (and non-edges) adjacent to it, then almost all queries exhibit high \emph{global sensitivity} (see Definition~\ref{def:GlobalSensitivity}). This is precisely why previous works either deal with fairly simple queries (such as degree profile~\cite{HayLMJ09}), or limit the change a single person can make to altering a single edge~\cite{nissim2007smooth, KRSY11, JLprivacy}. 

More importantly, previous works deal only with the relationship aspect of a social network, modeling it merely as a graph. However, a social network is composed also of different types of individuals (and perhaps even different types of relationships), each with her own attributes. As a result, the set of \emph{predicate queries} is much richer and much more sensitive when dealing with social networks. Indeed, in a standard database, a single person who changes her own attributes affects the number of people who \emph{are} spies by no more than $1$. In contrast, should Justin Beiber join the CIA then the number of people in Facebook who \emph{are friends with} a spy might increase dramatically.

Our work addresses these difficulties by introducing the notion of \emph{restricted sensitivity}. We postulate a set $\mathcal{H}$ that our input belongs to, and now we measure the sensitivity of a query only w.r.t databases in $\mathcal{H}$. This allows us to restrict the set of inputs \emph{for which we provide good utility guarantees} to a subset of ``nice'' inputs. In general, we map a query $f$ to an alternative query $f_{\cal H}$ s.t. $f$ and $f_{\cal H}$ identify over the inputs in ${\cal H}$, yet the global sensitivity of $f_{\cal H}$ is much small than the global sensitivity of $f$. Therefore, the mechanism that answers according to $f_{\cal H}$ and adds Laplace random noise preserves privacy for \emph{all} inputs, while giving good estimations of $f$ for nice inputs.

While our general scheme for devising such $f_{\cal H}$ is non-efficient and requires that we devise an independent $f_{\cal H}$ for each query $f$, we also design a complementary \emph{projection-based} approach. A projection of $\mathcal{H}$ is a function mapping all inputs to inputs of $\mathcal{H}$ with the property that any input in $\mathcal{H}$ is mapped to itself. Therefore, a projection $\mu$ allows us to define $f_{\cal H}$ for any $f$, simply by composing $f_{\cal H} = f\circ \mu$. However, in order to privately answer $f$ while adding only a fairly small amount of noise to each element of $\mathcal{H}$, we must have that $\mu$ satisfies certain properties, which we define in Section~\ref{sec:Results}. Informally, these properties imply smoothness of the projection or smoothness of the distance between an input and its projected image.

Motivating the projection approach is the definition of nice graphs as graphs with max-degree $k$. This could be explained as leveraging prior belief regarding the social network in question. For example, a study on the anatomy of Facebook \cite{ugander2011anatomy} shows that the maximum degree of any node in the graph is at most $k=5000$ whereas the number of nodes is about $9\cdot 10^8$. As we show, while computing a projection for each possible graph is not polynomial-time tractable, we devise a tractable approximate-projection scheme. Details are also in Section~\ref{sec:Results}.

We study two types of queries in connection with graphs of bounded max degree: subgraph counting (e.g. how many triangles involve at least two spies?) and predicates (e.g. how many people know two spies who don't know each other?). By using the framework of restricted sensitivity, it is possible to preserve differential privacy for both types of queries by adding a fairly small random noise to the true answer, in comparison with either the standard approach or the smooth-sensitivity approach of~\cite{nissim2007smooth}. This is due to the fact we \emph{refine the granularity} of the answer for the former type, and \emph{decrease the sensitivity} of the latter type. Our results are summarized in Tables~\ref{table:Results} and~\ref{table:NoiseLevel}. 
\textbf{TO REMOVE THIS NEXT SENTENCE.} 
Interestingly, in Appendix~\ref{?} we exhibit that a large set of queries that can be answered in more general model(arbitrary change to a vertex), even without using restricted sensitivity. Provided that the graph contains sufficiently many nodes, we show that one can implement all graph property-testers in a differential privacy preserving manner.

\begin{table}
\centering
  \begin{tabular}{ | l || c | c | c | c | c | }
\hline  & Adjacency & Hypothesis & Query  & Sensitivity   & Efficient   \\ \hline Theorem
\ref{thm:ConstructFprime} & Any & Any & Any & $GS_{f_{\cal H}} = RS_f\paren{\cal H}$ & No  \\ \hline Theorem
\ref{thm:ConstructFprimeEfficient} & Edge  & ${\cal H}_k$ & Any & $GS_{f_{\cal H}} = 3 RS_f\paren{\cal H}$ & Yes  \\ \hline
Theorem \ref{thm:main} & Vertex  & ${\cal H}_k$ & Any & $LS_{f_{\cal H}} = O\paren{1}\times RS_f\paren{{\cal H}_{2k}}$ & Yes  \\ \hline
\end{tabular} \caption{Summary of Results} \label{table:Results}
\end{table}

\begin{table}
\centering
\begin{tabular}{ | l || p{.7in} |
p{.7in} | p{.7in} | p{.7in} | } \hline  & \multicolumn{2}{c|}{Subgraph Counting
Query $P$} &       \multicolumn{2}{c|}{Local Profile Query}  \\ \hline
Adjacency  & Smooth  & Restricted    & Smooth  & Restricted  \\ \hline Edge  &
$O\paren{n^{|P|-1} }$ & $O\paren{k^{|P|-1}}$ & $O(n)$ & $O(k)$ \\ \hline Vertex
& $O\paren{k^{|P|-1}}$ & $O\paren{k^{|P|-1}}$ & $O(n)$ & $O(k)$ \\ \hline
\end{tabular} \caption{Sensitivity:  $G \in {\cal H}_k$}   \label{table:NoiseLevel} \end{table}

{\noindent \bf Organization.} Next we examine related work. Preliminary
definitions can be found in Section \ref{sec:preliminaries}. In Section
\ref{sec:restriced_sensitivity} we introduce the notion of restricted sensitivity and detail the general, non-efficient, construction of $f_{\cal H}$. Efficient projection-based schemes, demonstrate for the specific case of graphs of bounded-degree are details in Section~\ref{sec:Results}. We define subgraph counting queries and local-profile queries in Section~\ref{sec:RestrictedSensitivity}, where we also analyze the restricted and smooth sensitivity of these queries. We conclude with open questions in Section \ref{sec:futureQuestions}.
\input{itcs_related}



==> itcs_open.tex <==
\section{Future Questions/Directions} \label{sec:futureQuestions}
We focused on the hypothesis $H_k$? What other natural hypthothesis could be used to restrict sensitivity? Could the notion of restricted sensitivity be used to answer multiple queries in a noninteractive setting (e.g., BLR \cite{Blum:2008:LTA:1374376.1374464})?


